Automatic State Interaction with Large Localized Active Spaces for Multimetallic Systems

The localized active space self consistent field (LASSCF) method factorizes a complete active space (CAS) wave function into an antisymmetrized product of localized active space wave function fragments. Correlation between fragments is then reintroduced through LAS state interaction (LASSI), in which the Hamiltonian is diagonalized in a model space of LAS states. However, the optimal procedure for defining the LAS fragments and LASSI model space is unknown. We here present an automated framework to explore systematically convergent sets of model spaces, which we call LASSI[$r$,$q$]. This method requires the user to select only $r$, the number of electron hops from one fragment to another and $q$, the number of fragment basis functions per Hilbert space, which converges to CASCI in the limit of $r,q\to\infty$. Numerical tests of this method on the tri-metal complexes [Fe(III)Al(III)Fe(II)($\mu_3$-O)]$^{6+}$ and [Fe(III)$_2$Fe(II)($\mu_3$-O)]$^{6+}$ show efficient convergence to the CASCI limit with 4-10 orders of magnitude fewer states.

==> Tables/Main/10_11_LASSI_exploration.tex <==
\begin{table}[]
\centering
\label{tab:J_10_11}
\begin{tabular}{|c|HccH|}
\hline
\multicolumn{5}{|c|}{$J$ coupling in cm$^{-1}$}\\\hline
\diagbox{$\nmax$}{$r$}&0&1&2&3\\
%\diaghead{\theadfont Diag ColumnmnHead II}{$r$}{$\nmax$}&\thead{0}&\thead{1}&\thead{2}&\thead{3}\\
   \hline
1  & 116.69 & 114.65 & 114.65 & 114.65 \\
2  & 116.69 & 100.75 & 100.73 & 100.73 \\
3  & 116.69 & 36.91  & 36.81  & 36.81  \\
4  & 116.69 & 4.17   & 3.85   & 3.85   \\
5  & 116.69 & -2.90  & -3.28  & -3.28  \\
6  & 116.69 & -2.90  & -3.43  & -3.43  \\
7  & 116.69 & -2.90  & -3.52  & -3.52  \\
8  & 116.69 & -2.90  & -3.58  & -3.58  \\
9  & 116.69 & -2.90  & -3.66  & -3.66  \\
10 & 116.69 & -2.90  & -3.71  & -3.71 \\\hline
\end{tabular}
\caption{Performance of LASSI[$r$,$\nmax$] $\forall\;r\in \{0,3\}$ and $\forall \;\nmax\in \{1,10\}$ in reproducing $J$ [Eq.\ (\ref{eq:yamaguchi})] predicted by CASCI(11e,10o) of the AlFe$_2$ MOF node . $J_{\text{LASSI}[0,\nmax]}=+116.69cm^{-1}\; \forall\; \nmax=\{1,10\}$. $J_{\text{LASSI}[2,\nmax]} \approx J_{\text{LASSI}[3,\nmax]} \;\forall\; \nmax=\{1,10\}$.   The LAS-CASCI reference value is -3.82 cm$^{-1}$. The total number of states for each calculation is reported in SI table II.\textcolor{red}{This is updated with new set of calculation.}}
\end{table}

==> Tables/Main/15_16_navg.tex <==
\begin{tabular}{c|c|c}
        \\
        \\
        Type of rootspace   & Space Table & $\bar{n}_{\mathcal{P}K}$\\\hline
        \raisebox{-.5\height}{\includegraphics[width=20mm]{Figures/Main/navg_structures/f0f0f0.png}} & $\begin{bmatrix} N^{(1)} & S^{(1)} \\ N^{(2)} & S^{(2)} \\ N^{(3)} & S^{(3)} \end{bmatrix}=\begin{bmatrix} 6&2 \\ 5&\frac{5}{2} \\ 5&\frac{5}{2} 
        \end{bmatrix}$ & $\begin{bmatrix} 0.0000 \\ 0.0000 \\ 0.0000  \end{bmatrix}$\\
        \raisebox{-.5\height}{\includegraphics[width=20mm]{Figures/Main/navg_structures/f-1f0f1.png}} & $\begin{bmatrix} N^{(1)} +1  & S^{(1)} -\frac{1}{2} \\ N^{(2)} & S^{(2)} \\ N^{(3)} -1 & S^{(3)} +\frac{1}{2} \end{bmatrix}$ &$\begin{bmatrix} 1.6199 \\ 0.0000 \\ 1.6391  \end{bmatrix}$\\
        \raisebox{-.5\height}{\includegraphics[width=20mm]{Figures/Main/navg_structures/f1f0f-1.png}} & $\begin{bmatrix} N^{(1)} -1 & S^{(1)} - \frac{1}{2} \\ N^{(2)} & S^{(2)} \\ N^{(3)} +1 & S^{(3)} -\frac{1}{2}\end{bmatrix}^*$&$\begin{bmatrix} 0.6247 \\ 0.0000 \\ 1.1715  \end{bmatrix}$\\
        \raisebox{-.5\height}{\includegraphics[width=20mm]{Figures/Main/navg_structures/f-1f1f0.png}} & $\begin{bmatrix} N^{(1)} -1 & S^{(1)} -\frac{1}{2}\\ N^{(2)}+1 & S^{(2)}-\frac{1}{2} \\ N^{(3)} & S^{(3)} \end{bmatrix}$&$\begin{bmatrix} 1.1850 \\ 2.0292 \\ 0.0000  \end{bmatrix}$\\
        \raisebox{-.5\height}{\includegraphics[width=20mm]{Figures/Main/navg_structures/f1f-1f0.png}} & $\begin{bmatrix} N^{(1)} -1 & S^{(1)}-\frac{1}{2} \\ N^{(2)}+1 & S^{(2)}-\frac{1}{2} \\ N^{(3)} & S^{(3)} \end{bmatrix}^*$&$\begin{bmatrix} 1.0478 \\ 0.9200 \\ 0.0000  \end{bmatrix}$\\
        \raisebox{-.5\height}{\includegraphics[width=20mm]{Figures/Main/navg_structures/f0f1f-1.png}} & $\begin{bmatrix} N^{(1)} & S^{(1)} \\ N^{(2)}-1 & S^{(2)}-\frac{1}{2} \\ N^{(3)}+1 & S^{(3)}-\frac{1}{2} \end{bmatrix}$&$\begin{bmatrix} 0.0000 \\ 1.1859 \\ 1.3974  \end{bmatrix}$\\
        \raisebox{-.5\height}{\includegraphics[width=20mm]{Figures/Main/navg_structures/f0f-1f1.png}} & $\begin{bmatrix} N^{(1)} & S^{(1)} \\ N^{(2)}+1 & S^{(2)}-\frac{1}{2} \\ N^{(3)}-1 & S^{(3)}-\frac{1}{2} \end{bmatrix}$&$\begin{bmatrix} 0.0000 \\ 1.4912 \\ 1.2294  \end{bmatrix}$\\
    \end{tabular}
    \caption{Summary table of LASSI[1,5](16e,15o) results for the Fe$_3$ system for different rootspaces. The first column denotes a pictorial representation of the rootspace, in which the charge on each iron is that after the electron is transferred in the direction of the arrow. The change in spin on each iron in the rootspace is shown in the 2nd column. The third column shows the average excitation number [$\bar{n}_{K\mathcal{P}}$, Eq.\ (\ref{eq:navg})] on each fragment in the given rootspace.}
    \label{fig:navg_rootspaces}


 % Since all rootspaces with different polarizations are roughly similar, we present the average $\bar{n}_{K\mathcal{P}}$, expressed as $\sum_\mathcal{P}\bar{n}_{K\mathcal{P}}$/$\sum_\mathcal{P}1$. \\
     % * Since Fe$^{2+}$ has two possible spin changes when electron moves, only the rootspaces where $S$ goes down by $\frac{1}{2}$ have significant contribution. Full description of all significant rootspaces is provided in SI table XIV.

==> Tables/SI/Entropy/10_11.tex <==
\begin{table}[]
\centering
\caption{Entropy for AlFeFe node with (11e,10o) active space for LASSI[1,5]. Fe$^{2+}$ in red and Fe$^{3+}$ in blue. $s_{K\mathcal{P}}$ is entropy for $K$th fragment in $\mathcal{P}$ rootspace. $q^\text{(avg)}$ is also provided for reference. 5 rootspaces are not shown due to low weights.}
\label{tab:my-table}
\begin{tabular}{c|>{\color{red}}c>{\color{blue}}c|>{\color{red}}c>{\color{blue}}c}
Rootspace  & \multicolumn{2}{c}{${s}_{\mathcal{P}K}$} & \multicolumn{2}{c}{$\bar{q}_{\mathcal{P}K}$} \\\hline
\multirow{5}{*}{\includegraphics[width=20mm]{Figures/SI/DiIron/f0f0.png}} 
& 0.00                & 0.00                & 0.00  & 0.00  \\
& 0.00                & 0.00                & 0.00  & 0.00  \\
& 0.00                & 0.00                & 0.00  & 0.00  \\
& 0.00                & 0.00                & 0.00  & 0.00  \\
& 0.00                & 0.00                & 0.00  & 0.00  \\\hline
\multirow{5}{*}{\includegraphics[width=20mm]{Figures/SI/DiIron/f-1f1.png}} 
& 0.77                & 0.77                & 0.87  & 1.87  \\
& 0.79                & 0.79                & 0.95  & 1.87  \\
& 0.79                & 0.79                & 0.99  & 1.87  \\
& 0.79                & 0.79                & 0.91  & 1.87  \\
&&&&\\\hline
\multirow{5}{*}{\includegraphics[width=20mm]{Figures/SI/DiIron/f1f-1.png}} 
& 1.03                & 1.03                & 1.20  & 1.11  \\
& 1.02                & 1.02                & 1.21  & 1.11  \\
& 1.02                & 1.02                & 1.21  & 1.12  \\
& 1.02                & 1.02                & 1.21  & 1.10  \\
&&&&\\\hline
\end{tabular}
\end{table}

==> Tables/SI/Entropy/20_11.tex <==
\begin{table}[]
\centering
\caption{Entropy for AlFeFe node with (11e,20o) active space with LASSI[1,15]. Fe$^{2+}$ in red and Fe$^{3+}$ in blue. $s_{K\mathcal{P}}$ is entropy for $K$th fragment in $\mathcal{P}$ rootspace. $q^\text{(avg)}$ is also provided for reference. Note that even though $n^\text{(avg)}$ can be really high, the entropy is close to 1. \textcolor{red}{updated}}
\label{tab:20_11_entropy}
\begin{tabular}{c|>{\color{red}}c>{\color{blue}}c|>{\color{red}}c>{\color{blue}}c}
Rootspace  & \multicolumn{2}{c}{${s}_{\mathcal{P}K}$} & \multicolumn{2}{c}{$\bar{q}_{\mathcal{P}K}$} \\\hline
\multirow{9}{*}{\includegraphics[width=20mm]{Figures/SI/DiIron/f-1f1.png}}
& 0.14 & 0.14 & 2.27 & 1.68 \\
& 0.82 & 0.82 & 2.09 & 2.14 \\
& 0.14 & 0.14 & 2.27 & 1.70 \\
& 0.82 & 0.82 & 2.10 & 2.14 \\
& 0.14 & 0.14 & 2.27 & 1.73 \\
& 0.82 & 0.82 & 2.10 & 2.15 \\
& 0.22 & 0.16 & 2.30 & 1.70 \\
& 0.14 & 0.14 & 2.27 & 1.72 \\
& 0.82 & 0.82 & 2.10 & 2.14 \\\hline
\multirow{5}{*}{\includegraphics[width=20mm]{Figures/SI/DiIron/f0f0.png}}
&0.00 & 0.00 & 0.00 & 0.00 \\
&0.00 & 0.00 & 0.00 & 0.00 \\
&0.00 & 0.00 & 0.00 & 0.00 \\
&0.00 & 0.00 & 0.00 & 0.00 \\
&0.00 & 0.00 & 0.00 & 0.00 \\\hline
\multirow{19}{*}{\includegraphics[width=20mm]{Figures/SI/DiIron/f-1f1.png}}&0.13 & 0.13 & 0.16 & 2.69 \\
& 0.13 & 0.13 & 0.16 & 2.69 \\
& 0.22 & 0.34 & 6.98 & 1.86 \\
& 0.00 & 0.00 & 0.02 & 1.83 \\
& 0.13 & 0.13 & 0.16 & 2.69 \\
& 1.01 & 0.92 & 5.66 & 1.20 \\
& 0.20 & 0.21 & 7.01 & 2.09 \\
& 0.00 & 0.06 & 0.02 & 1.72 \\
& 0.13 & 0.13 & 0.16 & 2.69 \\
& 0.00 & 0.00 & 0.02 & 1.75 \\
& 0.22 & 0.25 & 6.98 & 2.24 \\
& 1.01 & 0.92 & 5.69 & 1.20 \\
& 0.13 & 0.13 & 0.16 & 2.69 \\
& 0.00 & 0.00 & 0.02 & 1.80 \\
& 0.24 & 0.37 & 6.88 & 2.28 \\
& 0.98 & 0.91 & 5.57 & 1.18 \\
& 0.13 & 0.13 & 0.16 & 2.69 \\
& 1.06 & 0.93 & 5.74 & 1.21 \\
& 0.13 & 0.13 & 0.16 & 2.69 \\\hline
\end{tabular}
\end{table}

==> Tables/SI/Figure_Data/10_11_heatmap.tex <==
\begin{table}

\begin{tabular}[c]{|c|c|c|ccccc|c|}
%\setlength{\LTcapwidth}{\textwidth}
\caption{Total Energy + 3971 $E_h$ for all states for various LASSI calculations with $r$ and $q$ and $J$ value with AlFe$_2$ with (11e,10o) active space.}
r                     & n    & States & S=9/2        & S=7/2        & S=5/2        & S=3/2        & S=1/2        & J      \\\hline
%\endfirsthead
%
%\multicolumn{9}{c}%
%{{\bfseries Table \thetable\ continued from previous page}} \\
%r                     & n    & States & S=9/2        & S=7/2        & S=5/2        & S=3/2        & S=1/2        & J      \\\hline
%\endhead
%
\multirow{10}{*}{r=0}&q=1& 5     & -0.792354 & -0.787569 & -0.783847 & -0.781189 & -0.779594 & 116.69 \\
 &q=2& 10    & -0.792354 & -0.787569 & -0.783847 & -0.781189 & -0.779594 & 116.69 \\
 &q=3& 15    & -0.792354 & -0.787569 & -0.783847 & -0.781189 & -0.779594 & 116.69 \\
 &q=4& 20    & -0.792354 & -0.787569 & -0.783847 & -0.781189 & -0.779594 & 116.69 \\
 &q=5& 25    & -0.792354 & -0.787569 & -0.783847 & -0.781189 & -0.779594 & 116.69 \\
 &q=6& 25    & -0.792354 & -0.787569 & -0.783847 & -0.781189 & -0.779594 & 116.69 \\
 &q=7& 25    & -0.792354 & -0.787569 & -0.783847 & -0.781189 & -0.779594 & 116.69 \\
 &q=8& 25    & -0.792354 & -0.787569 & -0.783847 & -0.781189 & -0.779594 & 116.69 \\
 &q=9& 25    & -0.792354 & -0.787569 & -0.783847 & -0.781189 & -0.779594 & 116.69 \\
 &q=10& 25    & -0.792354 & -0.787569 & -0.783847 & -0.781189 & -0.779594 & 116.69 \\\hline
 \multirow{10}{*}{r=1}&q=1& 18    & -0.792354 & -0.787674 & -0.783994 & -0.781369 & -0.779817 & 114.65 \\
 &q=2& 52    & -0.792354 & -0.788224 & -0.785009 & -0.782712 & -0.781336 & 100.75 \\
 &q=3& 102   & -0.792354 & -0.790834 & -0.789668 & -0.788841 & -0.788318 & 36.91  \\
 &q=4& 168   & -0.792354 & -0.792213 & -0.792078 & -0.791969 & -0.791898 & 4.17   \\
 &q=5& 250   & -0.792354 & -0.792507 & -0.792598 & -0.792647 & -0.792671 & -2.90  \\
 &q=6& 290   & -0.792354 & -0.792507 & -0.792598 & -0.792647 & -0.792671 & -2.90  \\
 &q=7& 330   & -0.792354 & -0.792507 & -0.792598 & -0.792647 & -0.792671 & -2.90  \\
 &q=8& 370   & -0.792354 & -0.792507 & -0.792598 & -0.792647 & -0.792671 & -2.90  \\
 &q=9& 410   & -0.792354 & -0.792507 & -0.792598 & -0.792647 & -0.792671 & -2.90  \\
 &q=10& 450   & -0.792354 & -0.792507 & -0.792598 & -0.792647 & -0.792671 & -2.90  \\\hline
 \multirow{10}{*}{r=2}&q=1& 38    & -0.792354 & -0.787676 & -0.783996 & -0.78137  & -0.779817 & 114.65 \\
 &q=2& 126   & -0.792354 & -0.788227 & -0.785013 & -0.782715 & -0.781339 & 100.73 \\
 &q=3& 264   & -0.792354 & -0.790836 & -0.789673 & -0.78885  & -0.788329 & 36.81  \\
 &q=4& 452   & -0.792354 & -0.792214 & -0.792089 & -0.791994 & -0.791932 & 3.85   \\
 &q=5& 690   & -0.792354 & -0.792509 & -0.792612 & -0.792677 & -0.792712 & -3.28  \\
 &q=6& 872   & -0.792354 & -0.79251  & -0.792618 & -0.792689 & -0.79273  & -3.43  \\
 &q=7& 1072  & -0.792354 & -0.79251  & -0.792621 & -0.792696 & -0.792739 & -3.52  \\
 &q=8& 1290  & -0.792354 & -0.79251  & -0.792623 & -0.792701 & -0.792746 & -3.58  \\
 &q=9& 1526  & -0.792354 & -0.79251  & -0.792626 & -0.792707 & -0.792754 & -3.66  \\
 &q=10& 1780  & -0.792354 & -0.79251  & -0.792628 & -0.792711 & -0.79276  & -3.71  \\\hline
 \multirow{10}{*}{r=3}&q=1& 62    & -0.792354 & -0.787676 & -0.783996 & -0.78137  & -0.779817 & 114.65 \\
 &q=2& 216   & -0.792354 & -0.788227 & -0.785013 & -0.782715 & -0.781339 & 100.73 \\
 &q=3& 462   & -0.792354 & -0.790836 & -0.789673 & -0.78885  & -0.788329 & 36.81  \\
 &q=4& 800   & -0.792354 & -0.792214 & -0.792089 & -0.791994 & -0.791932 & 3.85   \\
 &q=5& 1230  & -0.792354 & -0.792509 & -0.792612 & -0.792677 & -0.792712 & -3.28  \\
 &q=6& 1610  & -0.792354 & -0.79251  & -0.792618 & -0.792689 & -0.79273  & -3.43  \\
 &q=7& 2038  & -0.792354 & -0.79251  & -0.792621 & -0.792696 & -0.792739 & -3.52  \\
 &q=8& 2514  & -0.792354 & -0.79251  & -0.792623 & -0.792701 & -0.792746 & -3.58  \\
 &q=9& 3038  & -0.792354 & -0.79251  & -0.792626 & -0.792707 & -0.792754 & -3.66  \\
 &q=10& 3610  & -0.792354 & -0.79251  & -0.792628 & -0.792711 & -0.79276  & -3.71  \\\hline
\multicolumn{2}{|c|}{CASCI}  & 52920  & -0.792354 & -0.792511 & -0.792632 &              & -0.792771 & -3.81\\ \hline
\end{tabular}
\label{tab:10_11_heatmap}
\end{table}

==> Tables/SI/Figure_Data/15_16_table.tex <==
\begin{table*}[]
\centering
\caption{Absolute energies for LASSI and LAS-CASCI upto 6 decimal digits in Fe$_3$ system with (16e,15o) active space.}
\label{tab:15_16_energies}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Spin   & LASSI[0,1]   & LASSI[1,1]   & LASSI[1,5]   & LASSI[1,5$_\text{CT}$] & LAS-CASCI    \\\hline
S=7 & -4992.234449 & -4992.234449 & -4992.234449 & -4992.234449 & -4992.234449 \\
S=6 & -4992.233872 & -4992.234049 & -4992.235012 & -4992.235012 & -4992.235015 \\
S=5 & -4992.233378 & -4992.233695 & -4992.235479 & -4992.235479 & -4992.235489 \\
S=4 & -4992.232966 & -4992.233392 & -4992.235854 & -4992.235854 & -4992.235871 \\
S=3 & -4992.232637 & -4992.233143 & -4992.236140 & -4992.236140 & -4992.236165 \\
S=2 & -4992.232127 & -4992.232597 & -4992.236344 & -4992.236344 & -4992.236376 \\
S=1 & -4992.231751 & -4992.232181 & -4992.236360 & -4992.236360 & -4992.236394 \\
S=0 & -4992.231511 & -4992.231869 & -4992.236311 & -4992.236311 & -4992.236345 \\\hline
States & 24           & 182          & 6910         & 3014          &  41.4 million           \\\hline
\end{tabular}
\end{table*}

==> Tables/SI/Figure_Data/30_16_table.tex <==


\begin{table*}[]
\centering
\caption{}
\label{tab:my-table}
\caption{(Absolute energies + 4992.36 $E_h$)$\times 100$ for LASSI and LAS-DMRGCI upto 6 decimal digits in Fe$_3$ system with (16e,30o) active space.}
\label{tab:30_16_energies}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
&\multicolumn{8}{c|}{LASSI}&\\\hline
Spin   & [0,1] & [1,1] &  [1,3$_\text{CT}$] & [1,4$_\text{CT}$] & [1,5$_\text{CT}$] & [1,6$_\text{CT}$] & [1,7$_\text{CT}$] & [1,8$_\text{CT}$] & DMRGCI \\\hline
7      & -0.5901  & -0.5942  & -0.5964 & -0.6269 & -0.6271 & -0.6287 & -0.6289 & -0.6290 & -0.6985 \\
6      & -0.5324  & -0.5382  & -0.5782 & -0.6841 & -0.6938 & -0.6965 & -0.6970 & -0.7001 & -0.7835 \\
5      & -0.4830  & -0.4901  & -0.5623 & -0.7300 & -0.7472 & -0.7509 & -0.7518 & -0.7580 & -0.8544 \\
4      & -0.4418  & -0.4500  & -0.5488 & -0.7648 & -0.7877 & -0.7924 & -0.7937 & -0.8031 & -0.9114 \\
3      & -0.4088  & -0.4178  & -0.5378 & -0.7893 & -0.8159 & -0.8219 & -0.8234 & -0.8363 & -0.9552 \\
2      & -0.3596  & -0.3712  & -0.5295 & -0.8050 & -0.8334 & -0.8408 & -0.8427 & -0.8591 & -0.9868 \\
1      & -0.3235  & -0.3167  & -0.5196 & -0.7846 & -0.8166 & -0.8245 & -0.8269 & -0.8453 & -0.9906 \\
0      & -0.3006  & -0.3088  & -0.5133 & -0.7597 & -0.7917 & -0.8007 & -0.8036 & -0.8246 & -0.9846 \\\hline
States & 24         & 380        & 3228      & 5720      & 8924      & 12840     & 17468     & 22808     &34 Trillion \\\hline             
\end{tabular}
\end{table*}

==> Tables/SI/Figure_Data/Rootspace_Navg.tex <==
\renewcommand\arraystretch{0.541}
\begin{longtable}
[c]{c|>{\color{red}}c>{\color{blue}}c>{\color{cadmiumgreen}}c|c|>{\color{red}}c>{\color{blue}}c>{\color{cadmiumgreen}}c|}
\caption{Average $q^\text{(avg)}$ for all roostpaces with considerable weights for LASSI[1,5] for Fe$_3$ with active space of (16e,15o). 24 rootspaces of the with no charge tranfer had $q^\text{(avg)}$ of less than $10^{-6}$ for all fragments. 134 out of 182 rootspaces are shown. Remaining 38 rootspaces have low weight and are omitted.}
\label{tab:rootspace_navg}\\
Rootspace Type              & $\Bar{q}_{\mathcal{P}0}$  & $\Bar{q}_{\mathcal{P}1}$& $\Bar{q}_{\mathcal{P}2}$& Rootspace Type              & $\Bar{q}_{\mathcal{P}0}$  & $\Bar{q}_{\mathcal{P}1}$& $\Bar{q}_{\mathcal{P}2}$  \\\hline
%\endfirsthead
%
%\endhead
%
\multirow{18}{*}{\includegraphics[width=20mm]{Figures/Main/navg_structures/f-1f0f1.PNG}} & 1.62 & 0.00 & 1.64 & 
\multirow{18}{*}{\includegraphics[width=20mm]{Figures/Main/navg_structures/f1f0f-1.PNG}}     & 0.63 & 0.00 & 1.17 \\
& 1.62 & 0.00 & 1.64 &                             & 0.63 & 0.00 & 1.17 \\
& 1.62 & 0.00 & 1.64 &                             & 0.64 & 0.00 & 1.17 \\
& 1.61 & 0.00 & 1.63 &                             & 0.63 & 0.00 & 1.17 \\
& 1.62 & 0.00 & 1.64 &                             & 0.63 & 0.00 & 1.17 \\
& 1.62 & 0.00 & 1.64 &                             & 0.63 & 0.00 & 1.17 \\
& 1.62 & 0.00 & 1.64 &                             & 0.63 & 0.00 & 1.17 \\
& 1.62 & 0.00 & 1.64 &                             & 0.63 & 0.00 & 1.16 \\
& 1.62 & 0.00 & 1.64 &                             & 0.63 & 0.00 & 1.18 \\
& 1.62 & 0.00 & 1.65 &                             & 0.63 & 0.00 & 1.17 \\
& 1.62 & 0.00 & 1.64 &                             & 0.63 & 0.00 & 1.16 \\
& 1.62 & 0.00 & 1.64 &                             & 0.63 & 0.00 & 1.17 \\
& 1.62 & 0.00 & 1.64 &                             & 0.63 & 0.00 & 1.18 \\
& 1.62 & 0.00 & 1.64 &                             & 0.63 & 0.00 & 1.16 \\
& 1.62 & 0.00 & 1.64 &                             & 0.63 & 0.00 & 1.17 \\
& 1.62 & 0.00 & 1.64 &                             & 0.57 & 0.00 & 1.20 \\
& 1.62 & 0.00 & 1.64 &                             & 0.63 & 0.00 & 1.17 \\
& 1.62 & 0.00 & 1.64 &                             & 0.63 & 0.00 & 1.17 \\\hline                        
\multirow{18}{*}{\includegraphics[width=20mm]{Figures/Main/navg_structures/f-1f1f0.PNG}}  & 1.20 & 2.03 & 0.00 &  
\multirow{18}{*}{\includegraphics[width=20mm]{Figures/Main/navg_structures/f1f-1f0.PNG}}  & 1.05 & 0.90 & 0.00 \\
& 1.15 & 2.01 & 0.00 &                             & 1.04 & 0.91 & 0.00 \\
& 1.20 & 2.03 & 0.00 &                             & 1.05 & 0.91 & 0.00 \\
& 1.19 & 2.03 & 0.00 &                             & 1.04 & 0.90 & 0.00 \\
& 1.18 & 2.02 & 0.00 &                             & 1.05 & 0.91 & 0.00 \\
& 1.15 & 2.01 & 0.00 &                             & 1.04 & 0.91 & 0.00 \\
& 1.18 & 1.96 & 0.00 &                             & 1.06 & 0.91 & 0.00 \\
& 1.19 & 2.03 & 0.00 &                             & 1.06 & 0.91 & 0.00 \\
& 1.18 & 2.02 & 0.00 &                             & 1.05 & 0.91 & 0.00 \\
& 1.18 & 2.02 & 0.00 &                             & 1.09 & 0.94 & 0.00 \\
& 1.18 & 2.02 & 0.00 &                             & 0.94 & 0.83 & 0.00 \\
& 1.18 & 2.02 & 0.00 &                             & 1.00 & 0.89 & 0.00 \\
& 1.18 & 2.02 & 0.00 &                             & 1.00 & 0.88 & 0.00 \\
& 1.17 & 2.01 & 0.00 &                             & 1.08 & 0.97 & 0.00 \\
& 1.18 & 2.02 & 0.00 &                             & 1.07 & 0.96 & 0.00 \\
& 1.18 & 2.02 & 0.00 &                             & 1.07 & 0.92 & 0.00 \\
& 1.18 & 2.02 & 0.00 &                             & 1.06 & 0.91 & 0.00 \\
& 1.18 & 2.02 & 0.00 &                             & 1.05 & 0.91 & 0.00 \\\hline
\multirow{19}{*}{\includegraphics[width=20mm]{Figures/Main/navg_structures/f0f-1f1.PNG}} & 0.00 & 1.46 & 1.23 &              \multirow{19}{*}{\includegraphics[width=20mm]{Figures/Main/navg_structures/f0f1f-1.PNG}}& 0.00 & 1.21 & 1.39 \\
& 0.00 & 1.50 & 1.23 &                             & 0.00 & 1.19 & 1.39 \\
& 0.00 & 1.50 & 1.23 &                             & 0.00 & 1.18 & 1.39 \\
& 0.00 & 1.51 & 1.23 &                             & 0.00 & 1.16 & 1.40 \\
& 0.00 & 1.51 & 1.23 &                             & 0.00 & 1.19 & 1.39 \\
& 0.00 & 1.46 & 1.23 &                             & 0.00 & 1.18 & 1.42 \\
& 0.00 & 1.50 & 1.23 &                             & 0.00 & 1.20 & 1.39 \\
& 0.00 & 1.50 & 1.23 &                             & 0.00 & 1.19 & 1.39 \\
& 0.00 & 1.50 & 1.23 &                             & 0.00 & 1.28 & 1.40 \\
& 0.00 & 1.50 & 1.2 &                             & 0.00 & 1.16 & 1.41 \\
& 0.00 & 1.50 & 1.23 &                             & 0.00 & 1.19 & 1.39 \\
& 0.00 & 1.48 & 1.23 &                             & 0.00 & 1.19 & 1.39 \\
& 0.00 & 1.48 & 1.22 &                             & 0.00 & 1.19 & 1.39 \\
& 0.00 & 1.50 & 1.23 &                             & 0.00 & 1.18 & 1.42 \\
& 0.00 & 1.51 & 1.23 &                             & 0.00 & 1.20 & 1.39 \\
& 0.00 & 1.45 & 1.23 &                             & 0.00 & 1.18 & 1.39 \\
& 0.00 & 1.50 & 1.23 &                             & 0.00 & 1.19 & 1.39 \\
& 0.00 & 1.50 & 1.23 &                             & 0.00 & 1.20 & 1.39 \\
& 0.00 & 1.50 & 1.23 &                             & 0.00 & 1.19 & 1.39 \\\hline


\end{longtable}

==> Tables/SI/Figure_Data/n_variation_plot.tex <==
\begin{table}
%\adjustbox{max width=\columnwidth}{...}
\begin{tabular}[c]{|c|c|c|ccccc|c|}
%\label{tab:alfe2-full}\\\hline
%AS              & 1,$n^\text{(max)}$ & States & S=9/2        & S=7/2        & S=5/2        & S=3/2        & S=1/2        & J     \\\hline
%\endfirsthead
%
%\multicolumn{9}{c}%
%{{\bfseries Table \thetable\ continued from previous page}} \\
AS               & LASSI[1,$q$]& States & S=9/2        & S=7/2        & S=5/2        & S=3/2        & S=1/2        & J      \\\hline
%\endhead
%
\multirow{6}{*}{(11,10)}&q=1& 18    & -0.792354 & -0.787674 & -0.783994 & -0.781369 & -0.77982 & 114.65 \\
 &q=2& 52    & -0.792354 & -0.788224 & -0.785009 & -0.782712 & -0.781336 & 100.75 \\
 &q=3& 102   & -0.792354 & -0.790834 & -0.789668 & -0.788841 & -0.788318 & 36.91  \\
 &q=4& 168   & -0.792354 & -0.792213 & -0.792078 & -0.791969 & -0.791898 & 4.17   \\
 &q=5& 250   & -0.792354 & -0.792507 & -0.792598 & -0.792647 & -0.792671 & -2.90  \\
 &\multicolumn{8}{c|}{$q=6$ to $q=10$ are same as $q=5$ upto 6 decimal points.}\\\cline{2-9}
 %&q=6& 290   & -0.792354 & -0.792507 & -0.792598 & -0.792647 & -0.792671 & -2.90  \\
 %&q=7& 330   & -0.792354 & -0.792507 & -0.792598 & -0.792647 & -0.792671 & -2.90  \\
 %&q=8& 370   & -0.792354 & -0.792507 & -0.792598 & -0.792647 & -0.792671 & -2.90  \\
 %&q=9& 410   & -0.792354 & -0.792507 & -0.792598 & -0.792647 & -0.792671 & -2.90  \\
 %&q=10& 450   & -0.792354 & -0.792507 & -0.792598 & -0.792647 & -0.792671 & -2.90  \\\cline{2-9}
 & CASCI         & 52920  &-0.792354 & -0.792511  & -0.792632 &              & -0.792771 & -3.81\\ \hline
\multirow{11}{*}{(9,9)} &q=1 & 13 & -0.792354 & -0.787678 & -0.7839990 & -0.7813737 & -0.779823 & 114.60 \\
&q=2  & 29  & -0.792354 & -0.788227 & -0.7850137 & -0.782718 & -0.781344 & 100.69 \\
&q=3  & 37  & -0.792354 & -0.790845 & -0.7896879 & -0.788868 & -0.788348 & 36.64  \\
&q=4  & 77 & -0.792354 & -0.792214 & -0.7920803 & -0.791972 & -0.791902 & 4.14   \\
&q=5  & 133 & -0.792354 & -0.792507 & -0.7925973 & -0.792646 & -0.792670 & -2.89  \\
% &\multicolumn{8}{c|}{$q=6$ to $q=10$ are same as $q=5$ upto 6 decimal points.}\\\hline
&q=6  & 165 & -0.792354 & -0.792507 & -0.792597 & -0.792646 & -0.792670 & -2.89  \\
&q=7  & 165 & -0.792354 & -0.792507 & -0.792597 & -0.792646 & -0.792670 & -2.89  \\
&q=8  & 165 & -0.792354 & -0.792507 & -0.792597 & -0.792646 & -0.792670 & -2.89  \\
&q=9  & 165 & -0.792354 & -0.792507 & -0.792597 & -0.792646 & -0.792670 & -2.89  \\
&q=10 & 165 & -0.792354 & -0.792507 & -0.792597 & -0.792646 & -0.792670 & -2.89  \\\cline{2-9}
& CASCI & 15876  & -0.792354 & -0.792511 & -0.792632 &              & -0.792770 & -3.81  \\\hline
\multirow{12}{*}{(11,20)} & q=1  & 33    & -0.891148 & -0.890886 & -0.890684 & -0.890539 & -0.890451 & 6.37  \\
&q=3  & 297   & -0.891157 & -0.890960 & -0.890808 & -0.890700 & -0.890632 & 4.80  \\
&q=5  & 825   & -0.891299 & -0.891212 & -0.891151 & -0.891111 & -0.891087 & 1.94  \\
&q=7  & 1617  & -0.891311 & -0.891239 & -0.891191 & -0.891161 & -0.891141 & 1.56  \\
&q=9  & 2673  & -0.891311 & -0.891299 & -0.891296 & -0.891297 & -0.891301 & 0.10  \\
&q=11 & 3993  & -0.891318 & -0.891320 & -0.891329 & -0.891338 & -0.891347 & -0.27 \\
&q=13 & 5577  & -0.891318 & -0.891389 & -0.891453 & -0.891503 & -0.891533 & -1.97 \\
&q=15 & 7425  & -0.891318 & -0.891462 & -0.891580 & -0.891666 & -0.891720 & -3.67 \\
&q=17 & 9537  & -0.891319 & -0.891467 & -0.891588 & -0.891678 & -0.891732 & -3.78 \\
&q=19 & 11913 & -0.891468 & -0.891468 & -0.891589 & -0.891678 & -0.891733 & -2.43 \\
&q=21 & 14553 & -0.891333 & -0.891528 & -0.891684 & -0.891799 & -0.891868 & -4.89\\\cline{2-9}
& CASCI& $6 \times 10^8$ &-0.891595 & -0.891848 &-0.892047 & -0.892191 &    -0.892278 & -6.245\\ \hline
\end{tabular}
\caption{Absolute energies + 3971 $E_h$ for various LASSI[$r=1$, $q$] and $J$ with AlFe$_2$ for (11e,10o), (9e,9o) and (11e,20o) active spaces. Note that (9e,9o) and (11e,10o) results are nearly identical, suggesting that the doubly occupied orbital is not contributing to the magnetic exchange coupling interaction.}
\end{table}

==> Tables/SI/Geometry/AlFeFe.tex <==
\begin{table}[]
\centering
\caption{Geometry of Al-Fe-Fe MOF Node. All values in $\AA$}
\label{tab:my-table}

\begin{tabular}{cccc}
O  & -2.220198244  & 0.3991903003  & 1.694471699   \\
O  & -1.685553245  & -1.782306322  & 1.431399507   \\
C  & -2.268517865  & -0.8319550379 & 1.983951274   \\
H  & -2.913342017  & -1.076728589  & 2.843786805   \\
O  & 1.388288081   & 2.079556156   & -1.347085675  \\
O  & -0.7599088595 & 2.580923635   & -0.849227704  \\
C  & 0.3465674686  & 2.753895325   & -1.438835699  \\
H  & 0.3723796145  & 3.61769966    & -2.12309115   \\
O  & 1.046960908   & -2.6425342    & 0.9613246722  \\
O  & -0.3991903003 & 2.220198244   & 1.694471699   \\
O  & 1.782306322   & 1.685553245   & 1.431399507   \\
C  & 0.8319550379  & 2.268517865   & 1.983951274   \\
H  & 1.076728589   & 2.913342017   & 2.843786805   \\
O  & -2.079556156  & -1.388288081  & -1.347085675  \\
O  & -2.580923635  & 0.7599088595  & -0.849227704  \\
C  & -2.753895325  & -0.3465674686 & -1.438835699  \\
H  & -3.61769966   & -0.3723796145 & -2.12309115   \\
Fe & -0.3798741893 & -1.792603363  & -0.2003377303 \\
O  & 0.6422231803  & -2.237796553  & -1.892914518  \\
Fe & 1.792603363   & 0.3798741893  & -0.2003377303 \\
O  & 2.237796553   & -0.6422231803 & -1.892914518  \\
O  & 2.6425342     & -1.046960908  & 0.9613246722  \\
Al & -1.236271642  & 1.236271642   & 0.350650148   \\
O  & -0.0449501954 & 0.0449501954  & 0.0127621413  \\
C  & 1.645528685   & -1.645528685  & -2.357112465  \\
H  & 2.056906298   & -2.056906298  & -3.294571292  \\
C  & 2.160924281   & -2.160924281  & 1.277584187   \\
H  & 2.796080543   & -2.796080543  & 1.918244302  
\end{tabular}
\end{table}

==> Tables/SI/Geometry/FeFeFe.tex <==
\begin{table}[]
\centering
\caption{Geometry of Fe-Fe-Fe MOF Node. All values in $\AA$}
\label{tab:Fe3_Geom}
\begin{tabular}{cccc}
O  & -1.396530536  & -2.155053668  & 1.497463409  \\
O  & -1.424929948  & -0.1579202181 & 2.556757216  \\
C  & -1.805663158  & -1.333357733  & 2.354770591  \\
H  & -2.611139824  & -1.698287377  & 3.015172572  \\
O  & 1.422169433   & -0.1727766066 & -2.448307975 \\
O  & 1.404243292   & -2.165442677  & -1.387375376 \\
C  & 1.812327533   & -1.345288486  & -2.246529164 \\
H  & 2.621336914   & -1.706173551  & -2.904090708 \\
O  & -1.428899418  & 2.343625706   & 1.186473538  \\
O  & -1.403562858  & -2.165307125  & -1.387572278 \\
O  & -1.422998602  & -0.1723629226 & -2.447964967 \\
C  & -1.812500488  & -1.345105901  & -2.246279414 \\
H  & -2.621699381  & -1.706195274  & -2.903496624 \\
O  & 1.425112371   & -0.1571948062 & 2.556693752  \\
O  & 1.397382095   & -2.154305543  & 1.497360669  \\
C  & 1.806221904   & -1.332524996  & 2.35469992   \\
H  & 2.611813123   & -1.697184248  & 3.015110605  \\
Fe & -0.0001429864 & 0.9716426461  & 1.624782043  \\
O  & 1.428198549   & 2.344050002   & 1.186026051  \\
Fe & -0.0001364224 & 0.952927878   & -1.522872889 \\
O  & 1.423595107   & 2.330128125   & -1.070103354 \\
O  & -1.423503945  & 2.330456754   & -1.069656998 \\
Fe & 0.0002549988  & -1.941619777  & 0.0458885284 \\
O  & -0.0001521382 & -0.0719149875 & 0.0721478962 \\
C  & 1.815220274   & 2.721515148   & 0.0544222441 \\
H  & 2.604057215   & 3.492625269   & 0.0488314748 \\
C  & -1.815568952  & 2.721425035   & 0.0548464944 \\
H  & -2.604489027  & 3.492449072   & 0.0492507598
\end{tabular}
\end{table}

==> Tables/SI/Orbitals/10_11.tex <==
\begin{table*}[]
\caption{LASSCF Optimized Active Space orbitals and their occupancies with the active space of (11e,10o). Isosurface value = 0.03. Note the shape of doubly occupied orbital. It is poorly defined, optimizing a fully filled or completely empty orbital is challenging since the energy is invariant to the rotation of those orbitals.}
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
\includegraphics[width=40mm]{Figures/SI/10_11/MO_MO101A.jpg}&\includegraphics[width=40mm]{Figures/SI/10_11/MO_MO102A.jpg}&\includegraphics[width=40mm]{Figures/SI/10_11/MO_MO103A.jpg}&\includegraphics[width=40mm]{Figures/SI/10_11/MO_MO104A.jpg} \\ 
2.0000&1.0000&1.0000&1.0000\\ \hline
\includegraphics[width=40mm]{Figures/SI/10_11/MO_MO105A.jpg}&\includegraphics[width=40mm]{Figures/SI/10_11/MO_MO106A.jpg}&\includegraphics[width=40mm]{Figures/SI/10_11/MO_MO107A.jpg}&\includegraphics[width=40mm]{Figures/SI/10_11/MO_MO108A.jpg}\\ 
1.0000&1.0000&1.0000&1.0000\\ \hline
&\includegraphics[width=40mm]{Figures/SI/10_11/MO_MO109A.jpg}&\includegraphics[width=40mm]{Figures/SI/10_11/MO_MO110A.jpg}&\\
& 1.0000&1.0000&\\ \hline
    \end{tabular}
    \label{tab:10_11_orbitals}
\end{table*}

==> Tables/SI/Orbitals/15_16.tex <==
\begin{table*}[]
\caption{LASSCF Optimized Active Space orbitals and their occupancies with the active space of (16e,15o). Isosurface value = 0.03}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\includegraphics[width=40mm]{Figures/SI/15_16/MO_MO105A.jpg}&\includegraphics[width=40mm]{Figures/SI/15_16/MO_MO106A.jpg}&\includegraphics[width=40mm]{Figures/SI/15_16/MO_MO107A.jpg}&\includegraphics[width=40mm]{Figures/SI/15_16/MO_MO108A.jpg}\\ 
2.0000&1.0000&1.0000&1.0000\\ \hline
\includegraphics[width=40mm]{Figures/SI/15_16/MO_MO109A.jpg}&\includegraphics[width=40mm]{Figures/SI/15_16/MO_MO110A.jpg}&\includegraphics[width=40mm]{Figures/SI/15_16/MO_MO111A.jpg}&\includegraphics[width=40mm]{Figures/SI/15_16/MO_MO112A.jpg}\\ 
1.0000&1.0000&1.0000&1.0000\\ \hline
\includegraphics[width=40mm]{Figures/SI/15_16/MO_MO113A.jpg}&\includegraphics[width=40mm]{Figures/SI/15_16/MO_MO114A.jpg}&\includegraphics[width=40mm]{Figures/SI/15_16/MO_MO115A.jpg}&\includegraphics[width=40mm]{Figures/SI/15_16/MO_MO116A.jpg}\\ 
1.0000&1.0000&1.0000&1.0000\\ \hline
\includegraphics[width=40mm]{Figures/SI/15_16/MO_MO117A.jpg}&\includegraphics[width=40mm]{Figures/SI/15_16/MO_MO118A.jpg}&\includegraphics[width=40mm]{Figures/SI/15_16/MO_MO119A.jpg}&\\
2.0000&1.0000&1.0000&\\ \hline
    \end{tabular}
    \label{tab:15_16_orbitals}
\end{table*}

==> Tables/SI/Orbitals/20_11.tex <==
\begin{table*}[]
\caption{LASSCF Optimized Active Space orbitals and their occupancies with the active space of (11e,20o). Isosurface value = 0.03}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO101A.jpg}&\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO102A.jpg}&\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO103A.jpg}&\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO104A.jpg}\\ 
1.98777&0.99658&0.99621&0.99601\\ \hline
\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO105A.jpg}&\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO106A.jpg}&\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO107A.jpg}&\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO108A.jpg}\\ 
0.99583&0.01195&0.00423&0.00406\\\hline
\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO109A.jpg}&\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO110A.jpg}&\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO111A.jpg}&\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO112A.jpg}\\ 
0.00389&0.00347&0.99789&0.99777\\\hline
\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO113A.jpg}&\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO114A.jpg}&\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO115A.jpg}&\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO116A.jpg}\\ 
0.99774&0.99772&0.99772&0.00228\\\hline
\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO117A.jpg}&\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO118A.jpg}&\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO119A.jpg}&\includegraphics[width=40mm]{Figures/SI/20_11/MO_MO120A.jpg}\\ 
0.00228&0.00226&0.00223&0.00211\\\hline
    \end{tabular}
    \label{tab:20_11_orbitals}
\end{table*}

==> Tables/SI/Orbitals/30_16.tex <==
\begin{table*}[]
\caption{LASSCF Optimized Active Space orbitals and their occupancies with the active space of (16e,30o). Isosurface value = 0.03}
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO105A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO106A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO107A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO108A.jpg}\\ 
1.98795&0.99659&0.99620&0.99605\\ \hline
\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO109A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO110A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO111A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO112A.jpg}\\ 
0.99581&0.01177&0.00423&0.00403\\\hline
\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO113A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO114A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO115A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO116A.jpg}\\ 
0.00390&0.00346&0.99790&0.99777\\\hline
\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO117A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO118A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO119A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO120A.jpg}\\ 
0.99774&0.99772&0.99772&0.00228\\\hline
\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO121A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO122A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO123A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO124A.jpg}\\ 
0.00228&0.00226&0.00223&0.00210\\\hline
\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO125A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO126A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO127A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO128A.jpg}\\ 
0.99790&0.99775&0.99773&0.99771\\ \hline
\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO129A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO130A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO131A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO132A.jpg}\\
0.99771&0.00229&0.00229&0.00227\\ \hline
&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO133A.jpg}&\includegraphics[width=40mm]{Figures/SI/30_16/MO_MO134A.jpg}&\\
&0.00225&0.00210&\\ \hline
    \end{tabular}
    \label{tab:30_16_orbitals}
\end{table*}

==> Tables/SI/Orbitals/9_9.tex <==
\begin{table*}[]
\caption{LASSCF Optimized Active Space orbitals and their occupancies with the active space of (9e,9o). Isosurface value = 0.03}
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
\includegraphics[width=40mm]{Figures/SI/9_9/MO_MO102A.jpg}&
\includegraphics[width=40mm]{Figures/SI/9_9/MO_MO103A.jpg}&
\includegraphics[width=40mm]{Figures/SI/9_9/MO_MO104A.jpg}&
\includegraphics[width=40mm]{Figures/SI/9_9/MO_MO105A.jpg}\\ 
1.0000&1.0000&1.0000&1.0000\\ \hline
\includegraphics[width=40mm]{Figures/SI/9_9/MO_MO106A.jpg}&
\includegraphics[width=40mm]{Figures/SI/9_9/MO_MO107A.jpg}&
\includegraphics[width=40mm]{Figures/SI/9_9/MO_MO108A.jpg}&
\includegraphics[width=40mm]{Figures/SI/9_9/MO_MO109A.jpg}\\ 
1.0000&1.0000&1.0000&1.0000\\ \hline
&\includegraphics[width=40mm]{Figures/SI/9_9/MO_MO110A.jpg}&&\\
& 1.0000&&\\ \hline
    \end{tabular}
    \label{tab:9_9_orbitals}
\end{table*}
